Level Set Restricted Voronoi Tessellation for Large scale Spatial Statistical Analysis

Spatial statistical analysis of multivariate volumetric data can be challenging due to scale, complexity, and occlusion. Advances in topological segmentation, feature extraction, and statistical summarization have helped overcome the challenges. This work introduces a new spatial statistical decomposition method based on level sets, connected components, and a novel variation of the restricted centroidal Voronoi tessellation that is better suited for spatial statistical decomposition and parallel efficiency. The resulting data structures organize features into a coherent nested hierarchy to support flexible and efficient out-of-core region-of-interest extraction. Next, we provide an efficient parallel implementation. Finally, an interactive visualization system based on this approach is designed and then applied to turbulent combustion data. The combined approach enables an interactive spatial statistical analysis workflow for large-scale data with a top-down approach through multiple-levels-of-detail that links phase space statistics with spatial features.

==> author.tex <==
% \author{Tyson Neuroth}
% \affiliation{%
%   \institution{University of California, Davis}
%   \streetaddress{1 Shields Ave.}
%   \city{Davis}
%   \state{CA}
%   \country{United States}}
% \email{taneuroth@ucdavis.edu}


\author{Tyson Neuroth, Martin Rieth, \textit{Member, IEEE}, Jacqueline H Chen, Konduri Aditya, and Kwan-Liu Ma}
\authorfooter{
\item
 Tyson Neuroth is with University of California, Davis. E-mail: taneuroth@ucdavis.edu.
}


% \author{Martin Rieth}
% \affiliation{%
%  \institution{Combustion Research Facility \\ Sandia National Laboratories}
%  \city{Livermore}
%  \state{CA}
%  \country{United States}}

% \author{Konduri Aditya}
% \affiliation{%
%   \institution{Indian Institute of Science}
%   \city{Bangalore}
%   \state{Karnataka}
%   \country{India}
% }

% \author{Jacqueline H Chen}
% \affiliation{%
%  \institution{Combustion Research Facility \\ Sandia National Laboratories}
%  \city{Livermore}
%  \state{CA}
%  \country{United States}}

% \author{Kwan-Liu Ma}
% \affiliation{%
%   \institution{University of California, Davis}
%   \streetaddress{1 Shields Ave.}
%   \city{Davis}
%   \state{CA}
%   \country{United States}}
% \email{ma@cs.ucdavis.edu}


==> sections/03-Methods-backup.tex <==
%\vspace{-2mm}

\input{sections/LRCVD}

\section{Methods}
\label{sec:methods}

First, we introduce a local statistical aggregation approach based on discrete, level-set restricted Voronoi tessellations. We describe the goals and properties of the approach, and the underlying algorithms and implementation. We then present a system and associated workflow for hierarchical spatial statistical analysis, and for pre-simulation analysis and configuration of the models and methods that may then be applied for in situ processing.

{\color{blue}
\subsection{Motivation and Research Challenge}

}

\subsection{Spatial Decomposition and Aggregation}


\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{images/f1.png}
  \vspace{-0.2in}
  \caption{A 2D case of the weighted centroidal Voronoi tessellation, where contours of one scalar field (shades of blue) impose the restrictions, and the second field (brown to green) controls the site density.}
  \vspace{-5mm}
  \label{fig:weighted2d}
\end{figure}

The purpose of our spatial decomposition is to segment the domain for local statistical aggregation of the underlying volumetric data. The high-level goals of our methodology are to (1) align the segmentation with the surfaces of a multiple nested level sets (2)  merge the segments into spatially coherent super-segments that can distributed cleanly through enclosing sets of contorted isosurfaces, (3) minimize the storage requirements while maintaining a satisfactory level of detail and statistical quality, and (4) compute the decomposition and statistical aggregations efficiently for large datasets.

\input{sections/ComponentBlockSampling}



\subsection{Centroidal Voronoi Tesselation}

A centroidal Voronoi tessellation (CVT) is a Voronoi tessellation where each Voronoi site point is at the centroid of the region it encapsulates. This is often achieved by iteratively computing each Voronoi cell's center of mass, and then re-positioning its site point to its centroid. The weighted centroid is analogous to the center of mass, which is defined discretely as $$\frac{1}{m(V_s)}\sum_{v \in V_s} m(v)\mathbf{x}(v)$$
where $V_s$ is the set of volume elements captured by the Voronoi site $s$, $\mathbf{m}(v)$ is the weighting function evaluated at volume element $v$, $\mathbf{x}(v)$ is the position vector of $v$, and $m(V_s)$ is the cumulative mass for all $v\in V_s$.

% \input{sections/GeodesicVoronoiDecomposition}

\subsection{Restricted and Weighted Centroidal Voronoi Tessellations}

Restricted weighted centroidal Voronoi tessellation is a natural choice to meet the first three goals. The restrictions force the decomposition to align to the level sets, and centroidal-ness, produces spatial regions optimized for regularity. The spatial cells also can be merged throughout the hierarchy: from the full domain to the level set's layers and their connected components, to within components as clusters of Voronoi cells. By ignoring data outside of the level set of interest, we also are also reducing the data significantly. And through weighting with an underlying saliency function, it is also possible to concentrate the density of Voronoi sites in more critical regions as to reduce the footprint. Figure~\ref{fig:weighted2d} shows an example of such an approach for a 2D auto-ignition simulation, where the level sets are based on one scalar (with blue contours),  while the site density is concentrated by using a second (brown to green). A small 3D weighted case is shown (top) based on the pressure field in a combustion simulation. 

% \input{sections/GeodesicallyWeightedCentroidalUpdating}


\subsection{Level Set Restricted Voronoi Decomposition}

However, when sandwiched between complex surfaces, a complicated problem arises. A normal centroidal Voronoi decomposition based on Euclidean distance will no longer be valid except in limiting cases where there is a requirement for a high site density around highly sharp features, or the algorithm will be subject to failure as sites are attracted by nearby voxels which are geodesically or topologically separated. 

\subsection{Geodesically Weighted Discrete CVT}
\label{sec:centroidal}

To overcome these obstacles, we propose a novel variation of the discrete CVT based on geodesic distances through discovered line of sight pathways with the curved spaces. The pathways are discovered by iteratively expanding the classifications from `line of sight' of existing ones, marking the boundaries between the now visible and invisible voxels as nodes, and adjusting each voxel's path back through the nodes to find the shortest ones. As we expand, we must cast rays from each location to determine of it can be expanded to at the given iteration from the existing sets of nodes. The way that the paths are formed can be thought of through an analogy where mirrors placed strategically throughout the curved spaces to allow light to reach a voxel to any Voronoi site from any other other through a series of reflections. 

Once all the voxels are mapped to their geodesically nearest Voronoi sites a centroidal updating scheme needs to evolve the distribution consistently, towards a a centroidal one according to the discrete geodesic path finding scheme. This poses a second challenge since a definition of the centroid is needed under this context, and a method of evolving the distribution towards them is also needed. The normal centroidal updating scheme can be described as moving each site to the center of mass of its Voronoi cell. However, the center of mass can be outside of the restrictions completely, \textit{e.g.} like a horse shoe. In our scheme, we can think instead of each voxel of the site's Voronoi cell as having a vote on where the site should move to next. In order to facilitate the ability of the sites to move around these curved and complex shapes, we only allow the voxels which are in a strait line of sight of it to cast votes. However, we propagate the votes of nodes outside of the line of site to the nearest ones inside the line of site, so that the voxels which connect those hidden voxels get more weight on their votes. Another way to visualize this, is as if the voxels outside of line of sight pull on the sites through a system of pulleys which weave through the domain around the obstacles.   

In the end, the Voronoi decomposition allows for a type of geodesic spacing and regularity that is suited for decomposing the volumetric bands of field data into coherent segments for later statistical aggregation.

% \subsubsection{Level Set Restricted Centroidal Voronoi Decomposition}
% \label{sec:centroidal}

% {\color{blue}
% \subsubsection{Notation}

% $S \subset \mathbb{R}^3$ represents the Voronoi sites positions $[ \mathbf{s}_1, \mathbf{s}_2, ..., \mathbf{s}_m]$, and $i_s$ represents the index of site $i$, while $I_s$ represents the indices for sites $0$ to $m$. Next we have the connected components $C \subset V$, which share the same notation for indexing.  Then we have the voxels $V$, with $i_v$ and $I_v$ representing the 1d flattened voxel indices for individual voxels and all of them respectively, while $i3_v$ and $I3_v$ denote their 3d indices. 

% Next, we have the maps $C(V) : V \longrightarrow C$, $C(S) : S \longrightarrow S$, $S(V) : V \longrightarrow S$, which represent voxels component memberships, the sites component memberships, and the voxels site memberships respectively.

% Then, we have $E(V) : V \longrightarrow {V,S}$, which represents the directed edge from a voxel to its source. In the context of this algorithm, each voxel eventually as one single source edge, which traces back to a single site. The length of this path is the geodesic distance from a site $v$ to $s$.  

% Then, we have $B(V) : V \longrightarrow \{0,1\}^8$, which maps each voxel to a bitset of size 8 where the 8 bits encode the state of voxel $v$. The $8$ state encoded are (1) whether voxels edge leads to a site or another voxel, (2) whether the voxel is active in a search at a given stage, (3) whether a voxel is resolved at a given stage, (4) whether the voxel is a source of another voxel or not. E.g., for some $v$ has the property if $\exists i \in I_e, E[i]=v$ And then we have $Q(V): V \longrightarrow \{-1, 0,...,26\}$ and $T : \{0,...,26\} \longrightarrow \{0,1,-1\}^3$ such that $Q(v_i)$ gives $-1$ if $v_i$ found no \textit{min neighbor}, and otherwise the index into $T$ such that $I3_{v_i} + T[ Q(V) ] = I3_{v_j}$ where the remapping $E(v_i) \longrightarrow E(E(v_j))$ gives a gives a shorter path from $v_i$ to $S(v_i)$} 

% Finally, we have the parameters of the algorithm, $M : V \longrightarrow m$ where $m_i$ is the mass of voxel $v_$, and $\gamma$, which is the attraction bias, such that $m^{\gamma}$ is the biased mass. And $\alpha$, which is the site density. These parameters combine to form the equation $|S(c_i)| = ...$    

% $\voxels$ represents the voxels site positions, $\sourcemap$ represents directed edges $u $, $STS$ is an array of bytes used as bitflags to track voxel states, $MNB$ is an array of bytes used to facilitate the communication between neighboring voxels, $\gamma$ is the attraction bias parameter which influences the forces of mass in weighted CVTs, $S_{\mu}$ is the set of moments sums for each site, $S_m$ arrays site masses, $M$ is the field used as mass for weighting a CVT, $D$ is the distances, $VC$ is the voxel component ids, and $SC$ is the site component ids.}

{\color{blue}
\subsection{Comparison with Alternative Methods}}

We describe the level set restricted case we tackle by $$v \in V_{s'} \iff s' = \min_{s\in S} d(v,s) \wedge L_c(v) = L_c(s)$$ where $L_c(v), L_c(s)$ identify which layer and connected component  $v$ and $s$ belong to. 

If each site is approximately convex, then one may simply define $d$ as the Euclidean distance. In the non-restricted case, convexity is guaranteed. However, with complex restrictions, this is not necessarily the case. This introduces a problem that must be solved since (1) the centroid of $s$ may be outside of $L_c(s)$ (as an analogy, the center of mass of a horseshoe), and (2) the mapping from volume elements to Voronoi sites is non-trivial since Euclidean distance may be invalid across boundaries. 

In other application areas, {\it e.g. } mesh refinement, surface reconstruction, and the construction of computational grids, it is important to avoid these problems by placing a sufficient concentration of site points around complex geometry. Recently, the first provably correct method for generating a conforming Voronoi tessellation around such manifolds has been discovered~\cite{abdelkader2020vorocrust}. 

However, when considering the goal of performing exploratory spatial statistical analysis, it is not a requirement for the tessellation to be support surface reconstruction. As the simplest argument, consider the un-tessellated layer between a pair of iso-surfaces. This is clearly a valid spatial region for statistical aggregation and analysis. To further decompose the domain one may subdivide this layer into 2, 3, or $n$ segments. The optimal quality of the subdivision is something that may be open to debate and depend on the application. But regularity in geodesic spacing is no doubt a useful for analysis of scientific data which is evolving according to highly contorted manifolds. We break the process of our method down into 3 parts, which are composed to form the full process, as shown in Algorithm:\ref{alg:1}. 
\vspace{0.07in}

{\color{blue}
\subsection{Role and Choice of Parameters}}

{\color{blue}
\subsection{Algorithm}}

\begin{figure*}
  \centering
  \includegraphics[width=0.99\linewidth]{images/steps.png}
  \caption{High level illustration of our CVT algorithm. Left to right, top to bottom: The scalar field, decomposing into layers based on a set of isosurfaces/contours, connected component labelling, component/block decomposition for stratified component sampling, heat map showing the mass of each segment which determines how many Voronoi sites to place in each segment, the seed Voronoi sites, geodesic distances from each voxel to its geodesically nearest site, the initial Voronoi tesselation, a centroidal update, lastly, the tesselation after multiple centroidal updates.}
  \vspace{-5mm}
  \label{fig:weighted2d}
\end{figure*}

\noindent
\textbf{Stratified Component-Wise Site Distribution.} Once the connected components have been computed, the task is to sample $n_c$ positions within each component $c$, where 

\centerline{$n_c = \frac{\alpha}{m(V)} \sum_{v\in c}m(v)^{\gamma}$ }
\noindent
and $\alpha$ is a parameter we term the \textit{site density}, and $\gamma$ is a parameter which we call the \textit{attraction} that can be varied to reduce or increase the effect of weighting. In the unweighted case this is a sampling of each component proportional to its volume. The process is illustrated in ~\ref{alg:2}. The process is done in parallel on the GPU using a stratification scheme which further subdivides components into blocks so that we can more evenly distribute. 
Afterwards we sum $m(C_b)$ for each block component as well as $m(C)$, the `mass`. Once  the net \textit{mass} of each block of each component is known, then the number of sites to place there is determined by the formula, $n_c = \frac{\alpha}{m(V)} \sum_{v\in c}m(v)^{\gamma}$. It is rounded up so each component has at least a one site. Next $n_c$ sites are distributed by initially providing each block the number it wholly deserves, $\floor{n_c \frac{m(C_b)}{m(C)}}$. Afterwards, any remaining, $n_l$. are optimally placed based on the underrepresented-ness of each $C_b$, based on: $$ur(C_b)=1.0 - \left( n{C_b}-n_c\frac{m(C_b)}{m(C)}\right).$$ The rest of the details are to be found in our source code.

\vspace{0.07in}

\noindent
\textbf{Discrete Geodesic Voronoi Decomposition.}
The next phase is to compute the CVT as detailed in Algorithm~\ref{alg:3}.
In the initial step, the nearest volume element to each site becomes a generator. Then, for each volume element $e$, we check its neighborhood. If a neighboring element $n(e)$ is active (meaning it has been assigned a Voronoi site), then we check the distance between $e$ and its neighbor's site, $d'=||\mathbf{x}(e)- \mathbf{x}(s(n(e)))||_2$. If this distance is shorter than the distance between $e$ and its site, $d(e, s(e))$, then next we check whether the line connecting $e$ and $s$ crosses a boundary by tracing a ray backwards from $e$ to $s$ and checking the component ids of the elements along the way. If no boundary is crossed then we set $s(e) = s(n(e))$ and $d(e, s)= ||\mathbf{x}(e)-\mathbf{x}(s(n(e)))||_2$.

Once the initial update converges, then we begin again with each volume element on the boundary by the seen and unseen voxels used as nodes by which new paths can connect, $e_{src}$, and the process is repeated as we set, $e_u$, to the sources $e_{src}$, such that $$||\mathbf{x}(e_{src})-\mathbf{x}(s(e_{src}))||_2 + ||(\mathbf{x}(e_u) - \mathbf{x}(e_{src})||_2$$ is minimal. This is done iteratively until the full space is `illumiated' and the sites cease to find shorter paths.

% The centroidal updating stage described is illustrated in ~\ref{alg:3}. The previously mentioned 8-bit array is reused to store the state of each volume element. The state of the volume elements that are beneath a site point is first initialized to the state \verb|RESOLVED|, and all others to the state \verb|NULL|. A const 8-bit offset array storing the 26 adjacent element offset directions $NB = [ (0,0,1), (0,0,-1)...(-1,-1,-1)]$ is used to represent the local neighborhood, and  another 8-bit array is used to store the \textit{min neighbor} of each element.

% The update steps are then performed on the neighborhoods of each \verb|RESOLVED| or \verb|ACTIVE| volume element in two stages. 

% In the first stage, a kernel parallelized over each volume element is used. For each neighbor that is \verb|ACTIVE| or \verb|RESOLVED|,  the distance to the site that the neighbor is mapped to is computed. If the distance is smaller than the current distance, then a check is made to ensure that the path from the current element to the Voronoi site that the neighbor is mapped to doesn't cross the boundary. To do this, we work backward, tracing a line towards it, and break if we encounter an element with a different component id. If the test succeeds, then  the elements \textit{min neighbor} value is set to the associated local index into $NB$ and its current distance to $d(e,s(n_e))$.


% In the next stage,  each element is inspected to determine if a \textit{min neighbor} was found, and if so,  the element's state is set to \verb|ACTIVE|, and its current site is set equal to the site of the \textit{min neighbor}.  

% The split into two stages is needed so that there are no race conditions in the states of the elements and their dependencies.

% This process is repeated until the point at which all of the unresolved elements in \textit{line of sight} of a Voronoi site are \verb|ACTIVE|, and each \verb|ACTIVE| element has no \textit{min neighbor}.

% The centroidal update is then processed for each site, based only on those \textit{line of sight} volume elements. This process is repeated until approximate convergence is reached when all Voronoi sites have stopped changing position within some threshold. The default threshold is $1.75d_v$ where $d_v$ is the unit length of a volume element.      


\begin{figure}
  \centering
  \includegraphics[width=0.9\linewidth]{images/geodesicUpdate2.png}
  \vspace{-0.15in}
  \caption{...}
  \vspace{-5mm}
  \label{fig:process}
\end{figure}

% \vspace{0.07in}


\noindent
\textbf{Geodesically Weighted Centroidal Update.}
The next component of the algorithm is the updating of the site positions. This is illustrated in $\ref{alg:4}$. In a GPU kernel parallelized over voxels, we sum the moments ($p_i \times m_i$, or mass times position) of each line of sight voxel captured for each Voronoi site. A Cuda Atomic add operator is used for the addition. The geodesic weighting comes into play as the line of sight voxels which are path nodes that connect voxels which are around corners are weighted by the amount of voxels that they're sources of. In other words, instead of \\

$$\mathbf{c}_s = \frac{1}{m(R_s)} \sum_{v\in{R_s}} m_v \mathbf{p}_v$$,
 
we compute

$$\mathbf{c}_s'= 
 \frac{1}{m(R_s)}\sum_{v\in R_s} m_v \mathbf{p}_{\phi(v)}, \text{ s.t. } \phi(v) = v \textbf{ \textit{if} } los(v) \textbf{ \textit{else} } \phi(src(v))$$
 
%  $$los(v)=false$$
 
 \noindent
 {{\scriptsize $L_s(R_s)$} are the line of sight voxels in the region of Voronoi site $s$.} This pushes the site towards the right direction for finding a position which balances the forces pulling on it from the different voxels in its domain throughout its myriad pathways around obstacles. However, it still doesn't guarantee that the geodesically weighted centroid $c'$ is valid. It can still run into a boundary. For this reason, we cast a ray towards the direction it was voted to move towards, and then stop at the moment it would otherwise hit the boundary, and then back off a few voxel lengths.

%\paragraph{Open Source Code}
%\label{sec:source}

%% We include the source code~\footnotetext{Source code for our CVT algorithm \url{https://anonymous.4open.science/r/LSRCVD}.} for the algorithms described.

\noindent
{\it Reduced Data and Ordered Layout.} 
Oftentimes, the level sets of interest will enclose only a subset of the full domain. For example, in combustion simulations, those level sets may be based on the distance function from the flame, and the bands of interest may be restricted to an overall small portion of the full data. In this case, it makes sense to use the level set as a means to extract a reduced subset of the data. After extracting this data, it is sorted hierarchically by level set and connected components before being written to disk. We also store the layer and component offsets into the layout, as shown in Figure~\ref{fig:hierarchy}. This provides a means to efficiently load individual layers or components, as each will be contiguous in storage. 
The total reduction in storage from discarding the regions beyond the layers can be approximated as $(n-r)\times (m+1) + n_l + n_c$ where $n$ is the number of volume elements in the full domain, $r$ is the size of the subset within the levels, and $m$ is the number of variables per volume element. $n_l$ and $n_c$ are the number of layers and components, respectively (for storing the offsets) which should be very small relative to $r$. Thus, when $(n-r)$ is large and or $m$ is large, the additional cost of storing coordinates becomes nearly negligible. In extreme-scale combustion simulations, $m$ can be greater than $100$, in which case the coordinates can be as little as $1\%$ of the total footprint of the reduced data. Beyond this, the various low footprint statistical summarization strategies that have been introduced by others in previous works can be applied for a further reduction, although these possibilities can be better understood through reading the literature.
\vspace{2mm}
\begin{figure}
  \centering
  \includegraphics[width=0.9\linewidth]{images/combined.png}
  \vspace{-0.2in}
  \caption{Top Right: The data layout is sorted hierarchically by layer and component. Middle right: (A) White line is a rough measure of geodesic distance based on paths along Voronoi cells following the level set restriction; blue line is Euclidean distance. (B) and (C) are two separate connected components of the same layer. Left: The tree view in our visualization system showing the iso-values defining the layers and the connected components as nodes. The grey nodes are designated as components that are too small to compare with statistical measures.}
  \vspace{-4mm}
  \label{fig:hierarchy}
\end{figure}

% \begin{figure}
%   \centering
%   \includegraphics[width=0.6\linewidth]{images/hierarchyStorage2.png}
%   \caption{The data layout sorted hierarchically by layer and component.}
%   \label{fig:hierarchy}
% \end{figure}

\vspace{-2mm}

\section{Interactive Visualization System}
\label{sec:vis}

To showcase our feature-based approach, we designed and implemented a prototype visualization system. The system represents one promising way that the dynamic spatial decomposition approach, introduced in Section~\ref{sec:centroidal}, could be leveraged. The system demonstrates the qualitative value of the approach, and we hope it can inspire more adaptations and ideas for similar work. Though beyond the scope of this work to present in detail, or with experimental results, we also offer our vision for a larger ecosystem that could utilize our work in Section~\ref{sec:future}.

The visualization workflow follows the natural hierarchical pattern for sub-selection that is implicit in spatial decomposition. As the user drills down into details, based on layers, connected components, Voronoi cells, smaller subsets of volume elements are brought into play for spatial statistical analysis. The layers, components, Voronoi sites, and volume elements are interacted on and visualized in 3 associated sets of views as shown in Figure.~\ref{fig:teaser}.  
Since the system is designed to support interactive multivariate statistical analysis, data from many fields may need to be active simultaneously. The hierarchical sub-selection becomes useful in this case, not only as a means to narrow down the features of interest, but also to improve performance since sub-selections at each level will significantly reduce the amount of active data.

{\color{blue}
\subsection{Motivation and Design Decisions}}

% \begin{figure}
%   \centering
%   \includegraphics[width=0.5\linewidth]{images/treeView.png}
%   \caption{The tree view in our visualization system, showing the iso-values defining the layers, and the connected components as nodes. The grey nodes are designated as components which are too small to compare with statistical measures.}
%   \label{fig:tree}
% \end{figure}

\subsection{Iso-Layers and Connected Components} The first set of views that the user will interact with are for selecting layers and their connected components. A tree-based visualization is used to show the nested hierarchy of connected components (Figure.~\ref{fig:hierarchy}). The set of components is also projected into a 2D view based on t-distributed stochastic neighbor embedding (t-SNE) (Figure.~\ref{fig:teaser} (Left). The projection is based on a pairwise distance matrix, which can use measures of statistical similarity, or other metrics. Similar components, dependent on the distance measure, will cluster together in the view. Components can be selected by the user through a lasso selection tool within the projection. Or alternatively, they can select by clicking the mouse on the nodes in the tree view. The selection mode may be set to one of 4 options: new selection, union, intersection, or set difference. These modes act as operators on the existing selection and the new selection. When a given mode is active, it is active in all of the plots at each level and thus there is a single set of buttons to engage these modes globally, as shown in Figure.~\ref{fig:teaser} in the upper left corner. 

Once a selection is made, the selected elements are highlighted in both views. In the projection view, the layer of each component is encoded using color. Since the layer is implicitly encoded in the tree view already, it is possible to encode other information on its nodes as well. As an example, in Figure.~\ref{fig:hierarchy}, color is used to encode $\mu_4(\ch{H_2O},p)$, which is the co-kurtosis of hydrogen mixture fraction and pressure. Since some components may contain too few samples, a threshold can be defined to suppress the encoding of the statistical metric. These components will instead be shown in gray. This helps to avoid false interpretation due to insufficient sample sizes and can be useful to highlight those smaller components which may be particularly meaningful to the scientist. For example, it may represent the emergence of a feature ({\it e.g. } the incipient development of an ignition event), or the onset of a feature disappearance. 

% \begin{figure}
%   \centering
%   \includegraphics[width=0.9\linewidth]{images/tsnefig.png}
%   \vspace{-0.15in}
%   \caption{Selecting different clusters with a t-SNE projection of the Voronoi sites. Top left: the selection of components (done with the lasso tool); middle and bottom left two plots: points representing Voronoi sites within the selected components and two instances where clusters have been selected and analyzed in the linked statistical plots (on the right).}
%   \vspace{-5mm}
%   \label{fig:tsne}
% \end{figure}

% \begin{figure}
%   \centering
%   \includegraphics[width=0.7\linewidth]{images/topo2.png}
%   \caption{(A) White line is a rough measure of geodesic distance based on paths along Voronoi cells following the level set restriction; blue line is Euclidean distance. (B) and (C) are two separate connected components of the same layer.}
%   \label{fig:topo}
% \end{figure}

\begin{figure*}
  \centering
  \includegraphics[width=0.95\linewidth]{images/figplots.png}
  \vspace{-0.1in}
  \caption{Several configurations of the generalized joint plot. Left: KDE plot, with sub-selection points (blue), conditional curves, and sub-marginals displayed. The arrow indicators on the histogram margins point out the range and distribution of the active data in reference to the enclosing super-set. Middle: the scatter plot layer is active, and the lasso tool has been used to select the points (blue). Right: the GMM layer is displayed.}
  \label{fig:jointPlot}
  \vspace{-0.2in}
\end{figure*}

\subsection{Voronoi Cell Views}

Upon selecting connected components the Voronoi cells within those components will become active and can then be selected based on their projections in the 2D t-SNE projections as shown in the middle right of Figure.~\ref{fig:teaser} and also in Figure.~\ref{fig:tsne}. The first projection is based on a statistical distance metric, while the other one uses a spatial similarity metric. In Figure.~\ref{fig:tsne}, the former is based on similarity in the joint distribution of $\ch{H_2O}$ and $\ch{OH}$, while in the latter, the projection is based on a customized spatial distance metric that combines Euclidean distance and approximate geodesic distance along the iso-layer. This is illustrated in Figure.~\ref{fig:hierarchy} (A). The blue line shows the Euclidean distance, while the white line shows geodesic distance. The rationale behind this distance metric is the need to detect the local condition where a surface (e.g. flame) has become highly folded. In combustion, for example, this may represent adjacent flame-flame interactions, as flame surfaces approach one another at distances less than a laminar flame thickness. The condition where the Euclidean distance between two Voronoi cells is small, yet the geodesic distance is large, can be used as a rough heuristic to detect these sorts of interactions, or their preconditions. The metric is defined mathematically as $$d(s_i, s_j) = \frac{\alpha ||\mathbf{x}(s_i) - \mathbf{X}(s_j)||_2}{ \min_{p\in P_{i,j}}L(p)}$$ for $i \neq j$ else $0$, where $P_{i,j}$ is the set of paths in the network of connected Voronoi site neighborhood, $L(p)$ is the distance of the minimum geodesic path, and $\alpha$ is a weighting parameter to tune how strongly the ratio affects similarity. With this measure, for a pair of Voronoi sites in the same component, if the Euclidean distance between them is small relative to their geodesic distance, then they will be placed nearby one another in the t-SNE projection. 


While the geodesic terms is a rough measure it is made efficient enough to be practical due to the reduced set of paths associated with the coarse grain Voronoi representation. To find the minimum path the connectivity of the Voronoi sites if first computed, and then Johnson's all-pairs shortest path algorithm (which internally uses Dijkstra's algorithm for each Voronoi pair) is used. The neighborhood is also restricted to within connected components which further reduces the computational cost. The computation is parallelized by letting different threads operate on different components. The  Boost graph library's implementation is used, which has time complexity $O(|V|\cdot |E| \cdot log (|V|))$, where $V$ is the set of nodes, and $E$ is the set of edges. An alternative to Johonson's/Dijkstra's is to use the Floyd-Warshall all pairs shortest path algorithm which has time complexity $O(|V|^3)$. However, since our network is only locally connected it is sparse enough that $O(|V| \cdot |E| \cdot log(|V|))$ is significantly better than $O(|V|^3)$.   

These two views interact in the same manner as the aforementioned component projection view. Figure.~\ref{fig:tsne} shows an example, where clusters are selected from a Voronoi t-SNE projection and visualized in a statistical view.  Once selections are made in this view, the final level of the hierarchy (volume elements) becomes active. 

% \begin{figure}
%   \centering
%   \includegraphics[width=0.7\linewidth]{images/moments.png}
%   \caption{The joint plot with the histogram layer, sub-selection layer, conditional curves, sub-marginals, and moments table activated.}
%   \vspace{-4mm}
%   \label{fig:moments}
% \end{figure}

\subsection{Interactive Joint Plots}

At the stage where the statistical level becomes active, a subset of raw volume elements pre-selected from the previous levels in the hierarchy is available. It is then possible to explore in detail the joint distributions and correlations between different fields, as well as the details of their internal variation and spatial associations. 

Based on the experience of the domain scientists the following statistical plots are chosen to be incorporated into the system: joint probability distribution functions (PDFs) and their marginals, joint cumulative distribution functions (CDFs), conditional plots (which estimate one variable conditioned on 1 or 2 others), and scatter plots. Conveniently, each of these plots can share the same axis with the same scaling. Therefore, we can switch between these options, or combine them interactively as different layers on a single generalized joint plot. 

In addition, because we have sub-selected the volume elements from the previous layers, we can show additional context by plotting that data as a background layer. In the joint space this is shown as a dark gray scatter plot, and in the marginals, as the 1D gray histograms as shown in Figure.~\ref{fig:jointPlot}. 

Since the user will make selections with the lasso or box selection tool of the raw data points, it is useful that they can zoom in and out easily to further isolate particular groupings, or single them out. Since the visualized plot is already a subset of a larger set, zoomed in to a potentially smaller range of values, it makes sense to use the marginals of the larger set as a reference point for zooming in, so that one can see where they are relative to the other levels and also as they zoom in to extract more detail. On the marginals, we place arrows that point out the visualized sub-range, and the user can zoom in or pan on the range in each axis independently by scrolling with the mouse/trackpad, or clicking dragging, respectively. Furthermore, this means that two marginal distributions per axis are available, one for the subset and one for the super-set. Therefore,  the subset marginals can be added in between as a heat map. These submarginals can also be turned on or off on each plot individually.

When making sub-selections, it is useful to switch to a scatter plot view where the elements are distinguishable. After a selection has been made data points are plotted on the top layer in blue as shown in Figure.~\ref{fig:jointPlot}. The selection is highlighted across all views. This layer can be toggled on or off individually per plot so that one can see past the occlusion if desired. Since the data points also have spatial coordinates, one can also render them in the 3D view by rendering their bounding surfaces.

For modeling and visualizing the PDFs, there are 3 options, kernel density estimation (KDE), histograms, or Gaussian mixture models (GMM's). The KDE plots are useful for capturing high-level detail and smoothness in the potentially nonlinear or complex underlying distributions. Histograms and GMM's are included as they are models which are useful for in situ statistical feature detection as well as data reduction. One use case of our system is as a pre-simulation analysis tool, where the potential in situ statistical methods can be tested, configured, and validated beforehand. A few examples of the generalized joint plot with different layers activated are shown in Figure.~\ref{fig:jointPlot}. 

As the user interacts with the data, the PDFs may be interactively recomputed as the data inputs and the data range changes. Since the KDE and GMM plots are often not able to be recomputed immediately at interactive  rates, the plot will automatically switch from KDE or GMM to a histogram for example, while zooming/panning is occurring.

While exploring it is useful to allow the plots to adjust interactively based on the user's aforementioned actions. However, at some point, it is useful to fix the parameters of the model and test the same model on other spatial regions or other data. Therefore, the plots can be set to a locked mode. In the locked mode, the current statistical layer is saved as a texture, and when zooming or panning, rather than recomputing, the texture is simply transformed through scaling and translation. 

\begin{figure}
  \centering
  \includegraphics[width=0.85\linewidth]{images/converg.pdf}
  \vspace{-0.2in}
  \caption{The convergence of mean $d_s$ over the number of geodesically weighted centroidal update steps, shown for 3 different site densities. The algorithm converges similarly in each case to low mean $d_s$ (less than $0.5$ voxel widths), very rapidly. The  continues to improve slightly over time with diminishing returns on the benefit for the cost.}
  \label{fig:convergence}
\end{figure}


As a means to optimize and evaluate the PDFs, we estimate how well they preserve the higher-order moments of the joint distribution, which are often used in the analysis of turbulent flows \cite{sreeni97,bennett2011}. The estimated higher-order moments ({\it e.g. } covariance, coskewness, and cokurtosis) of the sample are compared against the population moments (computed from the raw data points). Each plot has a button that can be pressed to open/close an attached table that is auto-generated as a \LaTeX document as shown in Figure.~\ref{fig:moments}. This functionality would also aid featurization in high-order moments-based anomaly detection algorithms to identify features of interest \cite{aditya2019,kolla2020}.

{\color{blue}
\subsection{System Configuration and Parameters}}

% \begin{figure}
%   \centering
%   \includegraphics[width=0.8\linewidth]{images/workflow3.png}
%   \vspace{-2mm}
%   \caption{The larger workflow that encompasses the present work.}
%   \label{fig:workflow}
% \end{figure}

% Once the user is happy with the parameters and has discovered a pattern that is expressed in the statistical models, they will then be prepared to apply the same models within an in situ workflow.


